Variational Bayes Estimation of Discrete-Margined Copula Models with Application to Time Series

We propose a new variational Bayes estimator for high-dimensional copulas with discrete, or a combination of discrete and continuous, margins. The method is based on a variational approximation to a tractable augmented posterior, and is faster than previous likelihood-based approaches. We use it to estimate drawable vine copulas for univariate and multivariate Markov ordinal and mixed time series. These have dimension $rT$, where $T$ is the number of observations and $r$ is the number of series, and are difficult to estimate using previous methods. The vine pair-copulas are carefully selected to allow for heteroskedasticity, which is a feature of most ordinal time series data. When combined with flexible margins, the resulting time series models also allow for other common features of ordinal data, such as zero inflation, multiple modes and under- or over-dispersion. Using six example series, we illustrate both the flexibility of the time series copula models, and the efficacy of the variational Bayes estimator for copulas of up to 792 dimensions and 60 parameters. This far exceeds the size and complexity of copula models for discrete data that can be estimated using previous methods.

==> defs_letter.tex <==
\setlength{\topmargin}{-0.75in}
\setlength{\textheight}{9.5in}
\setlength{\oddsidemargin}{0pt}
%\textwidth 440pt 
\setlength{\textwidth}{6.5in}%width for US letterhead paper 
\parskip 0pt
\newcounter{num}
\newcommand{\utilde}[1]{\mathrel{\mathop{#1}\limits_{\displaystyle \widetilde{}}}}
%\def\baselinestretch{1.22}
\def\theequation{\thesection.\arabic{equation}}  
\def\abstract{\if@twocolumn
\section*{Abstract}
\else \normalsize 
\begin{center}
{\bf Summary\vspace{-.5em}\vspace{0pt}} 
\end{center}
\quotation 
\fi}
\def\endabstract{\if@twocolumn\else\endquotation\fi}
\newcommand{\bfy}{\mbox{{\bf y}}}
\newcommand{\bfw}{\mbox{\boldmath $w$}}
\newcommand{\bfs}{\mbox{\boldmath $s$}}
\newcommand{\bfg}{\mbox{\boldmath $g$}}
\newcommand{\bfu}{\mbox{\boldmath $u$}}
\newcommand{\bfv}{\mbox{\boldmath $v$}}
\newcommand{\bfx}{\mbox{\boldmath $x$}}
\newcommand{\bfzero}{\mbox{{\bf 0}}}
\newcommand{\bfalpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\bfmu}{\mbox{\boldmath $\mu$}}
\newcommand{\bff}{\mbox{{\bf f}}}
\newcommand{\bfb}{\mbox{{\bf b}}}
\newcommand{\bfone}{\mbox{{\bf 1}}}
\newcommand{\bfZ}{\mbox{\boldmath $Z$}}
\newcommand{\bfe}{\mbox{{\bf e}}}
\newcommand{\bfr}{\mbox{{\bf r}}}
\newcommand{\bfz}{\mbox{{\bf z}}}
\newcommand{\told}{\mbox{{\tiny old}}}
\newcommand{\tnew}{\mbox{{\tiny new}}}
\newcommand{\gammanew}{\mbox{$\gamma^{\tnew}$}}
\newcommand{\gammajnew}{\mbox{$\gamma^{\tnew}_j$}}
\newcommand{\gammaold}{\mbox{$\gamma^{\told}$}}
\newcommand{\gammajold}{\mbox{$\gamma^{\told}_j$}}
\newcommand{\zetan}{\mbox{$\zeta^{\tnew}$}}
\newcommand{\zetao}{\mbox{$\zeta^{\told}$}}
\newcommand{\phin}{\mbox{$\phi^{\tnew}$}}
\newcommand{\phio}{\mbox{$\phi^{\told}$}}
\newcommand{\phitn}{\mbox{$\tilde \phi^{\tnew}$}}
\newcommand{\phito}{\mbox{$\tilde \phi^{\told}$}}
\newcommand{\bfJ}{\mbox{\boldmath $J$}}
\newcommand{\bfpsi}{\mbox{\boldmath $\psi$}}
\newcommand{\bfepsilon}{\mbox{\boldmath $\epsilon$}}
\newcommand{\bfgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\bfbeta}{\mbox{\boldmath $\beta$}}
\newcommand{\bfomega}{\mbox{\boldmath $\omega$}}
\newcommand{\bfkappa}{\mbox{\boldmath $\kappa$}}
\newcommand{\bftheta}{\mbox{\boldmath $\theta$}}
\newcommand{\half}{\mathop{\frac{1}{2}}}
\newcommand{\var}{\mathop{\rm var}} 
\newcommand{\Exp}{\mathop{\rm E}}
\newcommand{\cov}{\mathop{\rm cov}}
\newcommand{\corr}{\mathop{\rm corr}}
\newcommand{\rank}{\mathop{\rm rank}}
\newcommand{\load}{\mbox{LOAD}}
\newcommand{\temp}{\mbox{TEMP}}
\newcommand{\hmd}{\mbox{HMD}}
\newcommand{\toy}{\mbox{TOY}}
\newcommand{\dum}{\mbox{DUM}}
\newcommand{\rowspace}{\mathop{\rm row~space}}
\makeatletter
\@addtoreset{equation}{section}
\makeatother
\newtheorem{lemma}{Lemma}[section]
\newtheorem{remark}{Remark}[section]
\newenvironment{Remark}{\begin{remark} \rm}{\end{remark}}
\newcommand{\myappendix}[1]{
%	\renewcommand{\thesection}{{\bf Appendix}~{\bf \Alph{section}}}
%	\section{#1}
	\setcounter{section}{1}
%	\renewcommand{\thesection}{\Alph{section}}} 
        \renewcommand{\thesection}{A\arabic{section}}}

\newcommand{\fah}[1]{
	\vspace{-0.2in}\nopagebreak
	\begin{center}
		{\sf -----#1-----}
	\end{center}\nopagebreak
	\vspace{-0.1in}}

\makeatletter
%% The "\@seccntformat" command is an auxiliary command
%% (see pp. 26f. of 'The LaTeX Companion,' 2nd. ed.)
\def\@seccntformat#1{\@ifundefined{#1@cntformat}%
   {\csname the#1\endcsname\quad}  % default
   {\csname #1@cntformat\endcsname}% enable individual control
}
\let\oldappendix\appendix %% save current definition of \appendix
\renewcommand\appendix{%
    \oldappendix
    \newcommand{\section@cntformat}{\appendixname~\thesection\quad}
}
\makeatother
\usepackage{cleveref} % just for this example




==> figs.tex <==
 \begin{figure}[H]
	\begin{center}
		\includegraphics[scale =1.1]{Figs/HomicideSeries.eps}
	\end{center}
	\caption{Time series plots and relative frequency histograms of the four univariate ordinal time series. The four rows correspond (from top to bottom) to the Murder, Attempted Murder, Manslaughter and Auto-Logistic examples.}
	\label{Fig:HomSeries}
\end{figure}


\begin{figure}[H]
	\begin{center}
		\includegraphics[scale =0.8]{Figs/Copulas9.eps}
	\end{center}
	\caption{Log-density functions of the pair-copulas at the MCMC posterior mean parameter values for the univariate copula models fit to the three crime series. Columns one to three correspond to the pair-copulas $c_2$, $c_3$ and $c_4$ respectively. Rows one to three correspond to Murder, Attempted Murder and Manslaughter, respectively}
	\label{Fig:Copulas9}
\end{figure}

%\begin{landscape}
\begin{figure}[H]
	\begin{center}
		\includegraphics[scale =1]{Figs/LowerBoundHomicideUnivariate.eps}
	\end{center}
	\caption{Variational lower bound values ${\cal L}(\bm{\lambda})$ for the VBDA estimators of the univariate time series copula models. From top to bottom, the rows correspond to the Murder, Attempted Murder, Manslaughter and Auto-Logistic examples. 
The first column plots  ${\cal L}$ at 
	the estimate of $\bm{\lambda}$, against the number of factors $K$ 
	in the factor decomposition  of $\Sigma$. 
   The second column plots  ${\cal L}$ against VB step for the case of $K=3$ factors. In each panel, 
   results are given for the
   VA1 (blue line), VA2 (red line) and VA3 (orange line) approximations.} 
	\label{Fig:LowerBound}
\end{figure}
%\end{landscape}

\begin{figure}[H]
	\begin{center}
		\includegraphics[scale =1.1]{Figs/VBvsMCMC.eps}
	\end{center}
	\caption{Comparison of the parameter 
		posterior means and standard deviations from the MCMC and VBDA methods for the 
		three crime count time series.  The first column compares the posterior means, while the second the posterior standard deviations. 
		Each row corresponds to a different crime series. VBDA was implemented with approximation VA2 and $K=3$ factors. Equivalent plots for VA1 and VA3 can be found in the Supplementary Material.}
		\label{Fig:VBvsMCMC}
\end{figure}

\begin{figure}[H]
	\begin{center}
		\includegraphics[scale =0.6]{Figs/LowerBoundHomicideMultivariate.eps}
	\end{center}
	\caption{Variational lower bound values ${\cal L}(\bm{\lambda})$ for the VBDA estimators of the  trivariate time series Homicide example. Panel~(a) plots ${\cal L}$ at 
		the estimate of $\bm{\lambda}$, against the number of factors $K$ in the
	 factor decomposition of $\Sigma$. 
    Panel~(b) plots ${\cal L}$ against VB step for the case of $K=15$ factors. In both panels 
    results are given for the
    VA1 (blue line), VA2 (red line) and VA3 (orange line) approximations.}
	\label{Fig:LowerBoundHomicideMultivariate}
\end{figure}

\begin{figure}[H]
	\begin{center}
		\includegraphics[scale =0.55]{Figs/Copulas12.eps}
	\end{center}
	\caption{Logarithm of the pair-copula densities computed at the VBDA posterior mean parameter values for the trivariate Homicide example. 
For each density, the superscript indicates the lag in the second argument of the pair-copula, while the subscript labels 1, 2 and 3 correspond to the Murder, Attempted Murder and Manslaughter count series, respectively. Results are given for variational approximation VA2 with $K=3$ factors.}
	\label{Fig:PairCopulasCrimeMulti}
\end{figure}


\begin{figure}[H]
	\begin{center}
		\includegraphics[scale =0.65]{Figs/BankuptcyTimeSeries.eps}
	\end{center}
	\caption{Panel (a) plots the bankruptcy count and VIX time series. The left vertical
		axis displays the number of bankruptcies, while the right vertical axis displays the VIX values. 
		Panel~(b) plots the density estimates of VIX, conditional on three ranges of values for 
		the number of bankruptcies. Denoting $B$ as the number of bankruptcies, the ranges
		 are $B<5$ (blue line density), $4<B<7$ (red line density) and $B>6$ (yellow line density).}
	\label{Fig:BankruptcySeries}
\end{figure}

\begin{figure}[H]
	\begin{center}
		\includegraphics[scale =0.5]{Figs/LowerBoundBankVIX.eps}
	\end{center}
	\caption{Variational lower bound values ${\cal L}(\bm{\lambda})$ for the VBDA estimators of the 
		bivariate time series of bankruptcy counts and VIX. Panel~(a) plots ${\cal L}$ at 
		the estimate of $\bm{\lambda}$, against the number of factors $K$ in the
		factor decomposition of $\Sigma$. 
		Panel~(b) plots ${\cal L}$ against VB step for the case of $K=15$ factors. In both panels 
		results are given for the
		VA1 (blue line), VA2 (red line) and VA3 (orange line) approximations.}
	\label{Fig:LowerBoundBankVIX}
\end{figure}






==> tabs.tex <==
\begin{table}[H]
	\centering
	\scalebox{1}{
		\begin{tabular}{lccccccc}
			\toprule
			             &       &         $\tau^a>0$          &         $\delta^a$          &         $\tau^b>0$          &         $\delta^b$          &             $w$             &      Kendall's $\tau$       \\ \cline{3-8}
			Murder       & $c_2$ &            0.141            &            0.313            &            0.219            &            0.523            &            0.743            &            0.065            \\
			             &       & ({\footnotesize0.04,0.34})  & ({\footnotesize 0.02,0.76}) & ({\footnotesize 0.01,0.81}) & ({\footnotesize 0.06,0.95}) & ({\footnotesize 0.22,0.99}) & ({\footnotesize 0.00,0.13}) \\
			             & $c_3$ &            0.161            &            0.610            &            0.190            &            0.516            &            0.782            &            0.097            \\
			             &       & ({\footnotesize 0.06,0.34}) & ({\footnotesize 0.14,0.97}) & ({\footnotesize 0.00,0.75}) & ({\footnotesize 0.06,0.95}) & ({\footnotesize 0.27,0.99}) & ({\footnotesize 0.03,0.17}) \\
			             & $c_4$ &            0.150            &            0.318            &            0.154            &            0.477            &            0.706            &            0.072            \\
			             &       & ({\footnotesize0.04,0.35})  & ({\footnotesize0.02,0.83})  & ({\footnotesize0.00,0.63})  & ({\footnotesize0.04,0.94})  & ({\footnotesize 0.22,0.99}) & ({\footnotesize 0.01,0.14}) \\ \cline{3-8}
			Attempted    & $c_2$ &            0.354            &            0.560            &            0.327            &            0.436            &            0.952            &            0.328            \\
			Murder       &       & ({\footnotesize0.27,0.43})  & ({\footnotesize 0.17,0.91}) & ({\footnotesize 0.01,0.89}) & ({\footnotesize 0.04,0.93}) & ({\footnotesize 0.84,0.99}) & ({\footnotesize 0.24,0.41}) \\
			             & $c_3$ &            0.227            &            0.771            &            0.232            &            0.541            &            0.876            &            0.180            \\
			             &       & ({\footnotesize 0.15,0.33}) & ({\footnotesize 0.46,0.98}) & ({\footnotesize 0.01,0.78}) & ({\footnotesize 0.07,0.95}) & ({\footnotesize 0.60,0.99}) & ({\footnotesize 0.12,0.25}) \\
			             & $c_4$ &            0.155            &            0.676            &            0.225            &            0.512            &            0.810            &            0.099            \\
			             &       & ({\footnotesize0.05,0.29})  & ({\footnotesize0.21,0.97})  & ({\footnotesize0.01,0.75})  & ({\footnotesize0.05,0.95})  & ({\footnotesize 0.33,0.99}) & ({\footnotesize 0.03,0.17}) \\ \cline{3-8}
			Manslaughter & $c_2$ &            0.195            &            0.484            &            0.208            &            0.491            &            0.628            &            0.052            \\
			             &       & ({\footnotesize0.03,0.50})  & ({\footnotesize 0.04,0.94}) & ({\footnotesize 0.01,0.69}) & ({\footnotesize 0.05,0.94}) & ({\footnotesize 0.12,0.97}) & ({\footnotesize-0.03,0.13}) \\
			             & $c_3$ &            0.173            &            0.389            &            0.224            &            0.524            &            0.688            &            0.061            \\
			             &       & ({\footnotesize 0.02,0.50}) & ({\footnotesize 0.03,0.90}) & ({\footnotesize 0.01,0.83}) & ({\footnotesize 0.07,0.96}) & ({\footnotesize 0.09,0.98}) & ({\footnotesize-0.01,0.14}) \\
			             & $c_4$ &            0.170            &            0.431            &            0.180            &            0.512            &            0.665            &            0.062            \\
			             &       & ({\footnotesize0.03,0.42})  & ({\footnotesize0.04,0.91})  & ({\footnotesize0.01,0.66})  & ({\footnotesize0.05,0.94})  & ({\footnotesize 0.14,0.98}) & ({\footnotesize-0.01,0.14}) \\ \bottomrule
		\end{tabular}}
	\caption{Posterior means of the pair-copula parameters for the D-vines fit to the three
		 univariate crime count time series, computed using MCMC data augmentation.
		 Each pair-copula is a mixture of two convex Gumbels, and the final column
		 reports the posterior mean of the overall Kendall's of each pair-copula.}
	\label{tab:ParEstimatesGumUnivariate}
\end{table}              

\begin{table}[H]
	\centering
	\begin{tabular}{lccc}
		\toprule
		                 &           $\rho_1$            &           $\rho_2$           &           $\rho_3$           \\ \midrule
		Murder           &             0.094             &            0.152**             &            0.128**             \\
		                 &  ({\footnotesize-0.01,0.19})  & ({\footnotesize 0.05,0.25})  & ({\footnotesize 0.03,0.22})  \\
		Attempted Murder &             0.458***             &            0.427***             &            0.382***             \\
		                 &  ({\footnotesize 0.34,0.56})  & ({\footnotesize 0.33,0.52})  & ({\footnotesize 0.28,0.48})  \\
		Manslaughter     &             0.057             &            0.073             &            0.076             \\
		                 & ({\footnotesize -0.026,0.14}) & ({\footnotesize -0.01,0.16}) & ({\footnotesize -0.00,0.16}) \\ \bottomrule
	\end{tabular}
	\caption{The posterior means of the pairwise Spearman correlations $\rho_k$,
		for $k = 1,2,3$, from the univariate time series copula models fit to the three
		monthly crime count time series. Correlations with approximate posterior intervals that do not contain zero
		at the 10\%, 5\% and 1\% level are denoted with `*', `**' and `***', respectively. The values are computed via simulation from the vine copula, as outlined in Section~\ref{sec:dts}.}
	\label{tab:spearmansCorrGumbel}
\end{table} 

\begin{table}
\centering
	{\small	
		\begin{tabular}{lccccccc}
			\toprule
			Example          &  Copula   &    No. of    &   No. of   & \multicolumn{3}{c}{Time VBDA} &  Time  \\
			                 & Dimension & Pair-Copulas & Parameters &   VA1   &  VA2   &    VA3     &  MCMC  \\ \midrule
			Murder           &    264    &      3       &     15     & 0.75 h  & 0.83 h &   2.30 h   &   h    \\
			Attempted Murder &    264    &      3       &     15     & 0.76 h  & 0.83 h &   2.32 h   &   h    \\
			Manslaughter     &    264    &      3       &     15     & 0.75 h  & 0.83 h &   2.32 h   &   h    \\
			Auto-Logistic    &    200    &      3       &     15     & 0.62 h  & 0.68 h &   1.53 h   & Failed \\
			Homicide         &    792    &      12      &     60     & 3.89  h & 4.10 h &            &  ---   \\
			Bankruptcy/VIX   &    658    &      9       &     45     &    h    &        &            &  ---   \\ \bottomrule
		\end{tabular}
}
	\caption{Copula model specifications and estimation times for the six examples. 
		The first four examples are univariate time series models, `Homicide' is the trivariate time
		series model in Section~\ref{sec:trivariateNSW}, and `Bankruptcy/VIX' is the bivariate time series model
		in Section~\ref{sec:vix}.
		The dimension of the D-vine copula, the number of unique pair-copulas, 
		and the number of unique copula parameters, are reported.  The total 
		times to estimate each model using our Matlab implementation (using 8 workers)
		are reported in hours. 
		The MCMC estimates are based on 30000 sweeps, 
		while the VBDA estimates are based on 5000 steps, $S = 500$ and $K=3/15$ for the 
		univariate/multivariate examples. 
		Computation times for MCMC estimation of the multivariate time series are excessive
		and unreported, while the MCMC sampler failed to converge for the Auto-Logistic example.}
		%The Markov order is three for the univariate models, one for the trivariate homicide model, and for the bivariate bankruptcy data is 2. 
	%For the $S$ evaluations of the copula density at each VB step, 32 parallel session were used in the Computational facility. 8000 VB steps
	\label{tab:timetable}
\end{table} 


%\begin{table}[H]
%	\centering
%	\scalebox{1}{
%		\begin{tabular}{lccccc}
%			\toprule
%			                 & \multicolumn{2}{c}{CRPS} & &\multicolumn{2}{c}{Log-Scores} \\ 
%			                 & Gumbel &        t        & &Gumbel  & t                    \\ \cline{2-3}\cline{5-6}
%			Murder           & 1.7035 &     1.7033      & &-2.5032 & -2.5017              \\
%			Attempted Murder & 1.7367 &     1.7337      & &-2.4691 & -2.4556              \\
%			Manslaughter     & 0.5782 &     0.5809      & &-1.3051 & -1.3063              \\ \bottomrule
%		\end{tabular}}
%	\caption{Log Scores}
%	\label{tab:LogScoresUnivarite}
%\end{table} 


	\begin{table}[H]
		\centering
		{\small
			\begin{tabular}{ccccccc}
				\toprule
				                          &              \multicolumn{6}{c}{D-Vine copula: $C^{MIX}$ with Convex Gumbel Components}               \\
				       Parameters         & $\tau^a>0$ & $\delta^a$ & $\tau^b>0$ & $\delta^b$ &  $w$  &                 Spearman                  \\ \midrule
				$\bm{\theta}_{1,2}^{(0)}$ &   0.200    &   0.548    &   0.347    &   0.507    & 0.929 & 0.169      {\footnotesize( 0.109,0.230)}  \\
				$\bm{\theta}_{1,3}^{(0)}$ &   0.084    &   0.395    &   0.118    &   0.499    & 0.617 & 0.020     {\footnotesize( -0.026,0.079)}  \\
				$\bm{\theta}_{2,3}^{(0)}$ &   0.153    &   0.656    &   0.167    &   0.496    & 0.785 & 0.093     {\footnotesize(  0.035,0.159)}  \\ \midrule
				$\bm{\theta}_{1,1}^{(1)}$ &   0.106    &   0.356    &   0.157    &   0.475    & 0.586 & 0.009     {\footnotesize( -0.055,0.073)}  \\
				$\bm{\theta}_{1,2}^{(1)}$ &   0.173    &   0.476    &   0.118    &   0.488    & 0.666 & 0.076     {\footnotesize(  0.014,0.154)}  \\
				$\bm{\theta}_{1,3}^{(1)}$ &   0.104    &   0.414    &   0.133    &   0.505    & 0.505 & -0.006     {\footnotesize( -0.070,0.055)} \\
				$\bm{\theta}_{2,1}^{(1)}$ &   0.205    &   0.706    &   0.167    &   0.482    & 0.842 & 0.154     {\footnotesize(  0.091,0.223)}  \\
				$\bm{\theta}_{2,2}^{(1)}$ &   0.341    &   0.623    &   0.220    &   0.474    & 0.932 & 0.306     {\footnotesize(  0.240,0.373)}  \\
				$\bm{\theta}_{2,3}^{(1)}$ &   0.153    &   0.499    &   0.110    &   0.528    & 0.528 & 0.023     {\footnotesize( -0.037,0.095)}  \\
				$\bm{\theta}_{3,1}^{(1)}$ &   0.130    &   0.476    &   0.097    &   0.477    & 0.512 & 0.012     {\footnotesize( -0.040,0.075)}  \\
				$\bm{\theta}_{3,2}^{(1)}$ &   0.172    &   0.417    &   0.143    &   0.485    & 0.698 & 0.084     {\footnotesize(  0.022,0.156)}  \\
				$\bm{\theta}_{3,3}^{(1)}$ &   0.150    &   0.555    &   0.136    &   0.498    & 0.568 & 0.028     {\footnotesize( -0.034,0.104)}  \\ \bottomrule
			\end{tabular}
		}
		\caption{The VBDA posterior means of the pair-copula parameters
			for the D-Vine copula fitted to the three-dimensional crime series using approximation VA2 and $K=15$ factors. 
			The posterior mean and 90\% probability intervals
			are also given for the
			Spearman's rho of each pair copula.
			Murder, Attempted Murder and Manslaughter counts
			are denoted
			as series 1, 2 and 3, respectively. Estimates for VA1 and VA3 are similar, and are given in the
			Supplementary Material.}
		\label{Tab:CopulaEstimatesCrimes}
	\end{table}


  
  
  
  
  
  
  
  
  
  
  
  


\begin{table}[H]
	\centering
	\scalebox{1}{
		\begin{tabular}{lcccc}
			\toprule
			                         &          Murder$_t$          &    Attempted Murder$_t$     &       Manslaughter$_t$       &  \\ \midrule
			\multicolumn{4}{l}{$\underline{k=0}$}                                                                                &  \\
			Attempted Murder$_t$     &           0.246***           &              -              &              -               &  \\
			                         & ({\footnotesize 0.16,0.33})  &                             &                              &  \\
			Manslaughter$_t$         &            0.055*            &          0.119***           &              -               &  \\
			                         & ({\footnotesize-0.01,0.13})  &  ({\footnotesize0.05,0.2})  &                              &  \\
			\multicolumn{4}{l}{$\underline{k=1}$}                                                                                &  \\
			Murder$_{t-1}$           &            0.071*            &          0.219***           &            0.028             &  \\
			                         & ({\footnotesize-0.02,0.17})  & ({\footnotesize0.12,0.33})  & ({\footnotesize-0.05,0.10})  &  \\
			Attempted Murder$_{t-1}$ &           0.221***           &          0.470***           &           0.089**            &  \\
			                         & ({\footnotesize 0.13,0.32})  & ({\footnotesize0.39,0.55})  & ({\footnotesize 0.01,0.18})  &  \\
			Manslaughter$_{t-1}$     &            0.015             &           0.104**           &            0.046             &  \\
			                         & ({\footnotesize -0.05,0.09}) & ({\footnotesize 0.03,0.19}) & ({\footnotesize -0.02,0.13}) &  \\ \bottomrule
		\end{tabular}}
	\caption{The VBDA estimates of the Spearman pairwise correlations $\rho_{i,j,k}$ for $k = 0,1$, using approximation VA2. The estimates of the posterior means are reported, with the 90\% posterior intervals below. These are computed from the copula model by simulation. 
	Correlations with approximate posterior intervals that do not contain zero
	at the 10\%, 5\% and 1\% level are denoted with `*', `**' and `***', respectively.}
	\label{tab:spearmansCorrGumbelMulti}
\end{table}      



\begin{table}[H]
	\centering
	\scalebox{1}{
		\begin{tabular}{lcc}
			\toprule
			                   &       Bankruptcy$_t$       &          VIX$_t$           \\ \midrule
			VIX$_t$            &          0.102***           &                            \\
			                   & ({\footnotesize 0.04,0.16}) &                            \\
			Bankruptcy$_{t-1}$ &          0.448***          &           0.075*           \\
			                   & ({\footnotesize0.37,0.52}) & ({\footnotesize-0.01,0.16}) \\
			VIX$_{t-1}$        &          0.200***          &          0.862***          \\
			                   & ({\footnotesize0.14,0.27}) & ({\footnotesize0.83,0.89}) \\
			Bankruptcy$_{t-2}$ &          0.334***          &           0.079*           \\
			                   & ({\footnotesize0.24,0.43}) & ({\footnotesize-0.02,0.18}) \\
			VIX$_{t-2}$        &          0.238***          &          0.740***          \\
			                   & ({\footnotesize0.16,0.31}) & ({\footnotesize0.67,0.80}) \\ \bottomrule
		\end{tabular}}
	\caption{The VB posterior means of the Spearman unconditional pairwise correlations $\rho_{i,j,k}$,
		for $k = 0,1,2$, computed from the copula model via simulation. Correlations with (variational) posterior intervals that do not contain zero
		at the 10\%, 5\% and 1\% level are denoted with `*', `**' and `***', respectively.}
	\label{tab:spearmansCorrGumbelMultiBankrutcy}
\end{table}          
    





   

==> web-append.tex <==
\noindent
\setcounter{page}{1}
%{\bf \Large{Online Appendix for `Copula Models of Serial Dependence
%for Heteroskedastic Time Series'
{\bf \Large{Online Appendix for `Variational Bayes Estimation of Discrete-Margined Copula Models with Application to Multivariate Ordinal and Mixed Time Series'
}}



\vspace{10pt}

\setcounter{figure}{0}
\setcounter{table}{0}
\renewcommand{\thetable}{A\arabic{table}}
\renewcommand{\thefigure}{A\arabic{figure}}
\noindent
This Online Appendix has two parts:
\begin{itemize}
	\item[] {\bf Part~A}: Provides additional empirical results for the VBDA fits two our multivariate and univariate time series examples.
	\begin{itemize}
		\item[] Table A2: 
		\item[] Table A3: 
		\item[] Table A4: 
		\item[] Table A5: 
		\item[] Figure A1: 
		\item[] Figure A2
	\end{itemize}
	\item[] {\bf Part~B}: Provides explanation and examples of the MATLAB code.

\end{itemize}
\newpage

\noindent {\bf \large{Part~A: Additional Empirical Results}}\\
\vspace{10pt}
	\begin{table}[H]
	\centering
	{\small
		\begin{tabular}{ccccccc}
			\toprule
			                          &               \multicolumn{6}{c}{D-Vine copula: $C^{MIX}$ with Convex Gumbel Components}                \\
			       Parameters         & $\tau^a>0$ & $\delta^a$ & $\tau^b>0$ & $\delta^b$ &  $w$  &                  Spearman                   \\ \midrule
			$\bm{\theta}_{1,2}^{(0)}$ &   0.200    &   0.591    &   0.323    &   0.500    & 0.917 & 0.167        {\footnotesize( 0.109,0.229)}  \\
			$\bm{\theta}_{1,3}^{(0)}$ &   0.078    &   0.428    &   0.114    &   0.496    & 0.604 & 0.014        {\footnotesize( -0.030,0.071)} \\
			$\bm{\theta}_{2,3}^{(0)}$ &   0.130    &   0.689    &   0.167    &   0.473    & 0.782 & 0.077        {\footnotesize(  0.025,0.139)} \\ \midrule
			$\bm{\theta}_{1,1}^{(1)}$ &   0.097    &   0.349    &   0.165    &   0.488    & 0.605 & 0.009        {\footnotesize( -0.055,0.071)} \\
			$\bm{\theta}_{1,2}^{(1)}$ &   0.165    &   0.486    &   0.122    &   0.479    & 0.663 & 0.072        {\footnotesize(  0.011,0.151)} \\
			$\bm{\theta}_{1,3}^{(1)}$ &   0.106    &   0.434    &   0.124    &   0.491    & 0.503 & 0.005        {\footnotesize(-0.065,0.051)}  \\
			$\bm{\theta}_{2,1}^{(1)}$ &   0.195    &   0.734    &   0.176    &   0.481    & 0.854 & 0.149        {\footnotesize(  0.088,0.216)} \\
			$\bm{\theta}_{2,2}^{(1)}$ &   0.336    &   0.690    &   0.193    &   0.489    & 0.924 & 0.299        {\footnotesize(  0.230,0.369)} \\
			$\bm{\theta}_{2,3}^{(1)}$ &   0.133    &   0.521    &   0.105    &   0.513    & 0.531 & 0.017        {\footnotesize( -0.037,0.086)} \\
			$\bm{\theta}_{3,1}^{(1)}$ &   0.126    &   0.489    &   0.095    &   0.468    & 0.497 & 0.010        {\footnotesize( -0.040,0.069)} \\
			$\bm{\theta}_{3,2}^{(1)}$ &   0.132    &   0.496    &   0.145    &   0.490    & 0.698 & 0.064        {\footnotesize(  0.008,0.135)} \\
			$\bm{\theta}_{3,3}^{(1)}$ &   0.139    &   0.564    &   0.124    &   0.501    & 0.564 & 0.026        {\footnotesize( -0.029,0.096)} \\ \bottomrule
		\end{tabular}
	}
	\caption{The VB posterior means of the pair-copula parameters
		for the D-Vine copula fitted to the three-dimensional crime series using approximation VA1. 
		The
		posterior mean and 90\% probability intervals
		are also given for the
		Spearman's rho of each pair copula.
		Murder, Attempted Murder and Manslaughter counts
		are denoted
		as series 1, 2 and 3, respectively.}
	\label{Tab:CopulaEstimatesCrimesVA1}
\end{table}

	\begin{table}[H]
	\centering
	{\small
		\begin{tabular}{ccccccc}
			\toprule
			                          &               \multicolumn{6}{c}{D-Vine copula: $C^{MIX}$ with Convex Gumbel Components}                \\
			       Parameters         & $\tau^a>0$ & $\delta^a$ & $\tau^b>0$ & $\delta^b$ &  $w$  &                  Spearman                   \\ \midrule
			$\bm{\theta}_{1,2}^{(0)}$ &   0.201    &   0.546    &   0.349    &   0.510    & 0.927 & 0.169        {\footnotesize( 0.111,0.230)}  \\
			$\bm{\theta}_{1,3}^{(0)}$ &   0.088    &   0.390    &   0.126    &   0.496    & 0.619 & 0.020        {\footnotesize(-0.027,0.079)}  \\
			$\bm{\theta}_{2,3}^{(0)}$ &   0.147    &   0.655    &   0.186    &   0.501    & 0.804 & 0.093        {\footnotesize( 0.039,0.153)}  \\ \midrule
			$\bm{\theta}_{1,1}^{(1)}$ &   0.103    &   0.353    &   0.163    &   0.480    & 0.594 & 0.008        {\footnotesize(-0.057,0.073)}  \\
			$\bm{\theta}_{1,2}^{(1)}$ &   0.175    &   0.475    &   0.119    &   0.487    & 0.661 & 0.076        {\footnotesize( 0.013,0.158)}  \\
			$\bm{\theta}_{1,3}^{(1)}$ &   0.105    &   0.412    &   0.142    &   0.505    & 0.513 & -0.006        {\footnotesize(-0.070,0.054)} \\
			$\bm{\theta}_{2,1}^{(1)}$ &   0.201    &   0.706    &   0.175    &   0.479    & 0.852 & 0.153        {\footnotesize( 0.094,0.217)}  \\
			$\bm{\theta}_{2,2}^{(1)}$ &   0.339    &   0.625    &   0.213    &   0.469    & 0.924 & 0.301        {\footnotesize( 0.232,0.372)}  \\
			$\bm{\theta}_{2,3}^{(1)}$ &   0.139    &   0.502    &   0.112    &   0.529    & 0.545 & 0.023        {\footnotesize(-0.037,0.094)}  \\
			$\bm{\theta}_{3,1}^{(1)}$ &   0.135    &   0.480    &   0.093    &   0.483    & 0.505 & 0.012        {\footnotesize(-0.038,0.073)}  \\
			$\bm{\theta}_{3,2}^{(1)}$ &   0.176    &   0.415    &   0.131    &   0.483    & 0.695 & 0.085        {\footnotesize( 0.024,0.159)}  \\
			$\bm{\theta}_{3,3}^{(1)}$ &   0.148    &   0.558    &   0.139    &   0.503    & 0.563 & 0.027        {\footnotesize(-0.037,0.107)}  \\ \bottomrule
		\end{tabular}
	}
	\caption{The VB posterior means of the pair-copula parameters
		for the D-Vine copula fitted to the three-dimensional crime series using approximation VA3. 
		The
		posterior mean and 90\% probability intervals
		are also given for the
		Spearman's rho of each pair copula.
		Murder, Attempted Murder and Manslaughter counts
		are denoted
		as series 1, 2 and 3, respectively.}
	\label{Tab:CopulaEstimatesCrimesVA3}
\end{table}

                                                    
                                                    
                                                    
                                                    
                                                    
                                                    
                                                    
                                                    
                                                    
                                                    
                                                    
                                                    

	\begin{table}[H]
	\centering
	{\small
		\begin{tabular}{ccccccc}
			\toprule
			                          &       \multicolumn{6}{c}{D-Vine copula: $C^{MIX}$ with Convex Gumbel Components}        \\
			       Parameters         & $\tau^a>0$ & $\delta^a$ & $\tau^b>0$ & $\delta^b$ &  $w$  &          Spearman           \\ \midrule
			$\bm{\theta}_{1,2}^{(0)}$ &   0.134    &   0.207    &   0.102    &   0.421    & 0.713 &            0.071           \\
			                          &            &            &            &            &       & {\footnotesize( 0.030,0.112)} \\ \midrule
			$\bm{\theta}_{1,1}^{(1)}$ &   0.360    &   0.870    &   0.326    &   0.491    & 0.940 &            0.321            \\
			                          &            &            &            &            &       & {\footnotesize( 0.259,0.384)} \\
			$\bm{\theta}_{1,2}^{(1)}$ &   0.122    &   0.458    &   0.121    &   0.544    & 0.608 &             0.032            \\
			                          &            &            &            &            &       & {\footnotesize(-0.017,0.101)} \\
			$\bm{\theta}_{2,1}^{(1)}$ &   0.191    &   0.232    &   0.107    &   0.470    & 0.814 &            0.139            \\
			                          &            &            &            &            &       & {\footnotesize( 0.095,0.184)} \\
			$\bm{\theta}_{2,2}^{(1)}$ &   0.719    &   0.693    &   0.241    &   0.509    & 0.979 &             0.699            \\
			                          &            &            &            &            &       & {\footnotesize( 0.662,0.734)} \\ \midrule
			$\bm{\theta}_{1,1}^{(2)}$ &   0.152    &   0.641    &   0.135    &   0.478    & 0.801 &             0.103            \\
			                          &            &            &            &            &       & {\footnotesize( 0.042,0.176)} \\
			$\bm{\theta}_{1,2}^{(2)}$ &   0.112    &   0.414    &   0.100    &   0.483    & 0.703 &            0.056            \\
			                          &            &            &            &            &       & {\footnotesize( 0.007,0.127)} \\
			$\bm{\theta}_{2,1}^{(2)}$ &   0.095    &   0.515    &   0.084    &   0.477    & 0.585 &            0.022            \\
			                          &            &            &            &            &       & {\footnotesize(-0.022,0.083)} \\
			$\bm{\theta}_{2,2}^{(2)}$ &   0.235    &   0.272    &   0.174    &   0.575    & 0.436 &           -0.009            \\
			                          &            &            &            &            &       & {\footnotesize(-0.079,0.057)} \\ \bottomrule
		\end{tabular}
	}
	\caption{The VB posterior means of the pair-copula parameters
		for the D-Vine copula fitted to the bankruptcy counts and VIX using approximation VA2. 
		The
		posterior mean and 90\% probability intervals
		are also given for the
		Spearman's rho of each pair copula.
		Bankruptcy counts and VIX
		are denoted
		as series 1 and 2, respectively.}
	\label{Tab:CopulaEstimatesBankruptcy}
\end{table} 


\begin{figure}[H]
	\begin{center}
		\includegraphics[scale =0.9]{Figs/AutoLog_paircop.eps}
	\end{center}
	\caption{Log-density function of the fitted pair-copulas at the variational posterior mean parameter values for the Auto-Logistic model. Rows one to three correspond to the pair-copulas $c_2$, $c_3$ and $c_4$ respectively. Columns one to three correspond to the approximations, VA1, VA2 and VA3, respectively.}
	\label{Fig:autologistic_paircop}
\end{figure}


\begin{figure}[H]
	\begin{center}
		\includegraphics[scale =1.1]{Figs/VBvsMCMCVA1.eps}
	\end{center}
	\caption{Comparison of the parameter 
		posterior means and standard deviations from the MCMC and VB methods
		for the copula models of each crime count time series. The first column compares the posterior means, while the second the posterior standard deviations. Each row corresponds to a different crime series.}
	\label{Fig:VBvsMCMCVA1}
\end{figure}

\begin{figure}[H]
	\begin{center}
		\includegraphics[scale =1.1]{Figs/VBvsMCMCVA3.eps}
	\end{center}
	\caption{Comparison of the parameter 
		posterior means and standard deviations from the MCMC and VB methods
		for the copula models of each crime count time series. The first column compares the posterior means, while the second the posterior standard deviations. Each row corresponds to a different crime series.}
	\label{Fig:VBvsMCMCVA3}
\end{figure}


\begin{figure}[H]
	\begin{center}
		\includegraphics[scale =0.58]{Figs/CopulasBankVix.eps}
	\end{center}
	\caption{Log-density function of the fitted pair-copulas at the MCMC posterior mean parameter values for the bivariate bankruptcy model. The super-index indicates the lagging in the second argument of the pair-copula, while the subscripts  1 and 2 correspond to the Bankruptcy and VIX variables, respectively.}
	\label{Fig:CopulasBankVix}
\end{figure}

\newpage
\noindent {\bf \large{Part~B: MATLAB code explanation and examples}}\\
\section*{Main functions}
\hrulefill \ \\
\texttt{VBDAfit\_uni}\hspace{1.5cm} \textit{Estimates copula models for univariate time series data using VBDA} \\
\hspace*{0.0001mm}\hrulefill
\ \\
\textbf{Inputs:}

\hspace{1.05cm}\texttt{y}\hspace{2cm} Data vector of dimension $T\times 1$.\\
\hspace*{1.7cm}\texttt{mdist}\hspace{1.1cm} MATLAB probability distribution object fitted to \texttt{y}.\\
\hspace*{1.7cm}\texttt{family}\hspace{0.9cm} Pair-copula family to use for D-Vine (only `gumbel\_mix' is available).\\
\hspace*{1.7cm}\texttt{p}\hspace{2cm} Markov order imposed on the D-Vine copula.\\
\hspace*{1.7cm}\texttt{k}\hspace{2cm} Number of factors in variational approximation.\\
\hspace*{1.7cm}\texttt{S}\hspace{2cm} Number of iterates used to compute gradient.\\
\hspace*{1.7cm}\texttt{nVB}\hspace{1.55cm} Total number of variational Bayes steps to be taken for inference.\\
\hspace*{1.7cm}\texttt{VA}\hspace{1.77cm} Selection of variational approximation. Set to 1 for VA1, to 2 for VA2 and \\ 
\hspace*{3.87cm}  to 3 for VA3.\\
\hspace*{1.7cm}\texttt{filename}\hspace{0.5cm} Optional MATLAB file name to export VBDA estimates. \texttt{filename} must end\\
\hspace*{3.85cm} with the extension \texttt{.mat} (\texttt{filename}=`example.mat'). If empty, no \texttt{.mat} file is\\
\hspace*{3.85cm} printed.\\
\ \\
\textbf{Outputs:} The function produces an object called \texttt{VBDAobj}. To call each argument use the format \texttt{VBDAobj.arg}, where \texttt{arg} can be either any of the input names, or the following:\ \\

\hspace{1.05cm}\texttt{gamma\_mean}\hspace{0.1cm} The variational posterior mean of the D-Vine copula parameters.\\
\hspace*{1.7cm}\texttt{gamma\_sd}\hspace{0.5cm} The variational standard deviation of the D-Vine copula parameters.\\
\hspace*{1.7cm}\texttt{mu}\hspace{1.75cm} Mean vector of approximation to the copula parameters distribution.\\
\hspace*{1.7cm}\texttt{B}\hspace{1.95cm} Factor matrix of the VB approximation covariance matrix.\\
\hspace*{1.7cm}\texttt{D}\hspace{1.95cm} Diagonal matrix of the VB approximation covariance matrix.\\
\hspace*{1.7cm}\texttt{muz}\hspace{1.55cm} For \texttt{VA=1} is empty. For \texttt{VA=\{2,3\}} is the vector with the means of the \\ \hspace*{3.85cm} variational approximation.\\
\hspace*{1.7cm}\texttt{logsigmaz}\hspace{0.2cm} For \texttt{VA=\{1,3\}} is empty. For \texttt{VA=2} is the vector with the logarithm of the \\ \hspace*{3.85cm} standard deviations of the variational approximation.\\
\hspace*{1.7cm}\texttt{C}\hspace{1.95cm} For \texttt{VA=\{1,2\}} is empty. For \texttt{VA=2} is the vector with the logarithm of the \\ \hspace*{3.85cm} standard deviations of the variational approximation.\\
\hspace*{1.7cm}\texttt{lambda}\hspace{0.85cm} Vector with all the variational parameters of the VBDA method.\\
\hspace*{1.7cm}\texttt{LB}\hspace{1.8cm} Lower bound at each VB step.
\ \\
\ \\
\hspace*{0.0001mm}\hrulefill \ \\
\texttt{VBDAfit\_multi}\hspace{1cm} \textit{Estimates copula models for multivariate time series data using VBDA} \\
\hspace*{0.0001mm}\hrulefill
\ \\
\textbf{Inputs:}

\hspace{1.05cm}\texttt{y}\hspace{2cm} Data matrix of dimension $T\times r$.\\
\hspace*{1.7cm}\texttt{type}\hspace{1.3cm} A MATLAB cell of size $1\times r$. Each element indicates if corresponding column\\ \hspace*{3.85cm} in \texttt{y}  is discrete or continuous. Set \texttt{type} to \texttt{`discrete'} or \texttt{`continuous'}.\\
\hspace*{1.7cm}\texttt{mdist}\hspace{1.1cm} A MATLAB cell of size $1\times r$, each element is a distribution object fitted to\\
\hspace*{3.85cm} corresponding column in \texttt{y}.\\
\hspace*{1.7cm}\texttt{family}\hspace{0.9cm} Pair-copula family to use for D-Vine (only `gumbel\_mix' is available).\\
\hspace*{1.7cm}\texttt{p}\hspace{2cm} Markov order imposed on the D-Vine copula.\\
\hspace*{1.7cm}\texttt{k}\hspace{2cm} Number of factors in variational approximation.\\
\hspace*{1.7cm}\texttt{S}\hspace{2cm} Number of iterates used to compute gradient.\\
\hspace*{1.7cm}\texttt{nVB}\hspace{1.55cm} Total number of variational Bayes steps to be taken for inference.\\
\hspace*{1.7cm}\texttt{VA}\hspace{1.79cm} Selection of variational approximation. Set to 1 for VA1, to 2 for VA2 and \\ 
\hspace*{3.88cm}  to 3 for VA3.\\
\hspace*{1.7cm}\texttt{filename}\hspace{0.5cm} Optional MATLAB file name to export VBDA estimates. \texttt{filename} must end\\
\hspace*{3.88cm} with the extension \texttt{.mat} (\texttt{filename}=`example.mat'). If empty, no \texttt{.mat} file is\\
\hspace*{3.88cm} printed.\\
\ \\
\textbf{Outputs:} The function produces an object called \texttt{VBDAobj}. To call each argument use the format \texttt{VBDAobj.arg}, where \texttt{arg} can be either any of the input names, or the following:\ \\

\hspace{1.05cm}\texttt{gamma\_mean}\hspace{0.1cm} The variational posterior mean of the D-Vine copula parameters.\\
\hspace*{1.7cm}\texttt{gamma\_sd}\hspace{0.5cm} The variational standard deviation of the D-Vine copula parameters.\\
\hspace*{1.7cm}\texttt{mu}\hspace{1.75cm} Mean vector of approximation to the copula parameters distribution.\\
\hspace*{1.7cm}\texttt{B}\hspace{1.95cm} Factor matrix of the VB approximation covariance matrix.\\
\hspace*{1.7cm}\texttt{D}\hspace{1.95cm} Diagonal matrix of the VB approximation covariance matrix.\\
\hspace*{1.7cm}\texttt{muz}\hspace{1.55cm} For \texttt{VA=1} is empty. For \texttt{VA=\{2,3\}} is the vector with the means of the \\ \hspace*{3.85cm} variational approximation.\\
\hspace*{1.7cm}\texttt{logsigmaz}\hspace{0.2cm} For \texttt{VA=\{1,3\}} is empty. For \texttt{VA=2} is the vector with the logarithm of the \\ \hspace*{3.85cm} standard deviations of the variational approximation.\\
\hspace*{1.7cm}\texttt{C}\hspace{1.95cm} For \texttt{VA=\{1,2\}} is empty. For \texttt{VA=2} is the vector with the logarithm of the \\ \hspace*{3.85cm} standard deviations of the variational approximation.\\
\hspace*{1.7cm}\texttt{lambda}\hspace{0.85cm} Vector with all the variational parameters of the VBDA method.\\
\hspace*{1.7cm}\texttt{LB}\hspace{1.75cm} Lower bound at each VB step.
\ \\
\ \\
\hspace*{0.0001mm}\hrulefill \ \\
\texttt{VBDApredict}\hspace{1.5cm} \textit{Generation from predictive densities of copula model} \\
\hspace*{0.0001mm}\hrulefill
\ \\
\textbf{Inputs:}

\hspace{1.05cm}\texttt{VBDAobj}\hspace{0.57cm} Object as produced by either function \texttt{VBDAfit\_uni} or \texttt{VBDAfit\_multi}.\\
\hspace*{1.7cm}\texttt{h}\hspace{1.92cm} Predictive horizon.\\
\hspace*{1.7cm}\texttt{n}\hspace{1.92cm} Number of draws.\\
\ \\
\textbf{Outputs:} \ \\

\hspace{1.05cm}\texttt{y\_pred}\hspace{1cm} A matrix of dimension $h\times r\times n$ with predictions from the copula model.\\
\ \\
\ \\
\hspace*{0.0001mm}\hrulefill \ \\
\texttt{VBDAspearman\_uni}\hspace{0.3cm} \textit{Spearman's correlations from fitted copula model for univariate times series} \\
\hspace*{0.0001mm}\hrulefill
\ \\
\textbf{Inputs:}

\hspace{1.05cm}\texttt{VBDAobj}\hspace{0.59cm} Object as produced by function \texttt{VBDAfit\_uni}.\\
\ \\
\textbf{Outputs:} \ \\

\hspace{1.05cm}\texttt{rhoSmean}\hspace{0.7cm} Posterior mean of pairwise Spearman's correlations.\\
\hspace*{1.7cm}\texttt{rhoSquant}\hspace{0.52cm} $5\%$ and $95\%$ quantiles of pairwise Spearman's correlations.\\
\ \\
\ \\
\hspace*{0.0001mm}\hrulefill \ \\
\texttt{VBDAspearman\_multi}\hspace{0.1cm} \textit{Spearman's correlations from fitted copula model for multivariate times series} \\
\hspace*{0.0001mm}\hrulefill
\ \\
\textbf{Inputs:}

\hspace{1.05cm}\texttt{VBDAobj}\hspace{0.57cm} Object as produced by function \texttt{VBDAfit\_multi}.\\
\ \\
\textbf{Outputs:} \ \\

\hspace{1.05cm}\texttt{rhoSmean}\hspace{0.7cm} Posterior mean of pairwise Spearman's correlations.\\
\hspace*{1.7cm}\texttt{rhoSquant}\hspace{0.52cm} $5\%$ and $95\%$ quantiles of pairwise Spearman's correlations.\\
\ \\
\ \\
\hspace*{0.0001mm}\hrulefill \ \\
\texttt{VBDAplots}\hspace{2cm} \textit{Summary plots from VBDA estimation} \\
\hspace*{0.0001mm}\hrulefill
\ \\
\textbf{Inputs:}

\hspace{1.05cm}\texttt{VBDAobj}\hspace{0.59cm} Object as produced by either function \texttt{VBDAfit\_uni} or \texttt{VBDAfit\_multi}.\\
\ \\
\textbf{Outputs:} This function produces three plots. 1) The data and the relative frequencies; 2) All the pair-copulas from the fitted D-Vine model; 3) The lower bound.
\newpage
\section*{Examples}
\subsection*{Example 1: Fitting Auto-Logistic example with binomial margin}
\lstinputlisting{Examples_uni.m}
\subsection*{Example 2: Fitting Homicide example with negative binomial margins}
\lstinputlisting{Examples_multi.m}


